The Geometry of Meaning in Neural Manifolds

Just as different languages express the same concept through different words, neural networks express similar functions through incompatible coordinate systems. Different architectures, random initializations, and optimization trajectories produce incompatible parameterizations in extrinsic coordinates, obscuring functional relationships between independently trained models. When models independently solve similar tasks on related data, do their learned representations share exploitable structure despite incompatible coordinates? This thesis shows that semantic correspondence is a fundamental primitive revealing shared geometric structure beneath incompatible parameterizations. By identifying which elements refer to the same semantic content, correspondence breaks the symmetry of arbitrary implementation choices, anchoring incompatible systems to a shared semantic frame and revealing the intrinsic geometry that enables zero-shot transformation between independently trained models. Building on this principle, fourteen contributions explore correspondence-based alignment across zero-shot model stitching, cross-modal translation, policy transfer, activation steering, and neural decoding. They span domains (vision, language, reinforcement learning, neuroscience), architectures (CNNs, Transformers, graph networks), and scales (from small supervised models to billion-parameter generative systems). Each exploits different geometric properties (angular, metric, spectral, sparse, or distributional), yet all instantiate the same principle. It extends beyond artificial systems: fMRI data show that different human brains processing identical stimuli exhibit alignable geometric structure. By revealing intrinsic geometric structure beneath extrinsic parameterization, semantic correspondence transforms model isolation into interoperability.

==> config/styling.tex <==

\usepackage[automake,symbols,abbreviations,nomain,nogroupskip]{glossaries-extra}
\newglossary*{concepts}{List of Concepts}
\makeglossaries

\glssetcategoryattribute{abbreviation}{regular}{true}
\glssetcategoryattribute{general}{regular}{true}
\glssetcategoryattribute{symbol}{regular}{true}

\newcommand\Chapter[2]{
  \chapter[#1]{#1\\\color{subtitlecolor}\medskip\large\itshape#2}
}

\setabbreviationstyle[withoutdesc]{short-long}
\setabbreviationstyle[withdesc]{short-long-desc}
\setabbreviationstyle[nolong]{short-nolong}

\input{glossaries/symbols}
\input{glossaries/abbreviations}

\addbibresource{bibliography/bibliography.bib}

\DeclareCiteCommand{\fullcite}
  {\usebibmacro{prenote}}
  {\defcounter{maxnames}{99}%
   \defcounter{minnames}{99}%
   \usedriver
     {\DeclareNameAlias{sortname}{default}}
     {\thefield{entrytype}}}
  {\multicitedelim}
  {\usebibmacro{postnote}}

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[chapter]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{assumption}[theorem]{Assumption}

\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{note}[theorem]{Note}


\newtcolorbox{publicationinfo}{
  enhanced,
  colback=black!3!white,
  colframe=black!40,
  boxrule=0.5pt,
  leftrule=3.5pt,
  arc=0pt,
  outer arc=0pt,
  left=12pt,
  right=12pt,
  top=10pt,
  bottom=10pt,
  before skip=1em,
  after skip=1em,
  borderline west={3.5pt}{0pt}{black!70}
}


==> glossaries/abbreviations.tex <==

\newabbreviation[category=withoutdesc, sort=rsa]{rsa}{RSA}{Representational Similarity Analysis}

\newabbreviation[category=withoutdesc, sort=llm]{llm}{LLM}{Large Language Model}

\newabbreviation[category=withoutdesc, sort=pca]{pca}{PCA}{Principal Component Analysis}

\newabbreviation[category=withoutdesc, sort=mlp]{mlp}{MLP}{Multi-Layer Perceptron}

\newglossaryentry{encoder}{
  type=concepts,
  name={Encoder},
  text={encoder},
  plural={encoders},
  description={The computational pathway from input to latent representation. For a classification network, the encoder comprises convolutional layers and pooling operations that produce feature representations. For a generative model, the encoder maps inputs to a latent bottleneck. For a language model, the encoder comprises the earlier layers that produce intermediate representations. See \Cref{ch:methodology}, \Cref{sec:neural-representations}.}
}

\newglossaryentry{decoder}{
  type=concepts,
  name={Decoder},
  text={decoder},
  plural={decoders},
  description={The computational pathway from latent representation to output. For a classification network, the decoder is the classification head mapping features to class logits. For a generative model, the decoder reconstructs outputs from latent codes. For a language model, the decoder comprises the later layers that process intermediate representations. See \Cref{ch:methodology}, \Cref{sec:neural-representations}.}
}

\newabbreviation[category=withoutdesc, sort=cnn]{cnn}{CNN}{Convolutional Neural Network}

\newabbreviation[category=withoutdesc, sort=ae]{ae}{AE}{AutoEncoder}

\newabbreviation[category=withoutdesc, sort=vae]{vae}{VAE}{Variational AutoEncoder}

\newabbreviation[category=withoutdesc, sort=linae]{linae}{LinAE}{Linear AutoEncoder}

\newabbreviation[category=withoutdesc, sort=linvae]{linvae}{LinVAE}{Linear Variational AutoEncoder}

\newabbreviation[category=withoutdesc, sort=relative]{relrep}{RelRep}{Relative Representations}

\newabbreviation[category=withoutdesc, sort=nlp]{nlp}{NLP}{Natural Language Processing}

\newabbreviation[category=withoutdesc, sort=cv]{cv}{CV}{Computer Vision}

\newabbreviation[category=withoutdesc, sort=cka]{cka}{CKA}{Centered Kernel Alignment}

\newabbreviation[category=withoutdesc, sort=cca]{cca}{CCA}{Canonical Correlation Analysis}

\newabbreviation[category=withoutdesc, sort=svcca]{svcca}{SVCCA}{Singular Value Canonical Correlation Analysis}

\newabbreviation[category=withoutdesc, sort=pwcca]{pwcca}{PWCCA}{Projection Weighted Canonical Correlation Analysis}

\newabbreviation[category=withoutdesc, sort=cos]{cos}{Cos.}{Cosine}

\newabbreviation[category=withoutdesc, sort=eu]{eu}{Eucl.}{Euclidean}

\newabbreviation[category=nolong, description={The MNIST dataset  \citep{Lecun1998-we}, a classic collection of handwritten digits widely used for training image processing systems.}, sort=mnist]{mnist}{MNIST}{MNIST}

\newabbreviation[category=withdesc, description={The Fashion MNIST dataset \citep{Xiao2017-er}, designed as a more complex alternative to the original MNIST, contains grayscale images of various fashion products.}, sort=fmnist]{fmnist}{F-MNIST}{Fashion MNIST}

\newabbreviation[category=nolong, description={The CIFAR-10 dataset \citep{Krizhevsky2009-hv}, composed of 60,000 32x32 color images in 10 classes, with 6,000 images per class.}, sort=cifar010]{cifart}{CIFAR-10}{CIFAR-10}

\newabbreviation[category=nolong, description={The CIFAR-100 dataset \citep{Krizhevsky2009-hv}, similar to CIFAR-10 but with 100 classes, providing a more challenging task for image classification models.}, sort=cifar100]{cifarh}{CIFAR-100}{CIFAR-100}

\newabbreviation[category=nolong, description={The ImageNet1k dataset \citep{deng2009imagenet}, a large-scale dataset designed for use in visual object recognition software research.}, sort=imagenet1k]{imagenet1k}{ImageNet1k}{ImageNet1k}

\newabbreviation[category=nolong, description={The Amazon Reviews dataset \citep{amazon-reviews}, a large collection of customer reviews, useful for sentiment analysis and other forms of Natural Language Processing.}, sort=amazon]{amazon}{Amazon Reviews}{Amazon Reviews}

\newabbreviation[category=nolong, description={The DBpedia dataset \citep{Auer2007-fb}, derived from Wikipedia, provides a structured form of Wikipedia's content for various knowledge extraction and semantic search tasks.}, sort=dbpedia]{dbpedia}{DBpedia}{DBpedia}

\newabbreviation[category=nolong, description={The N24News dataset \citep{wang-EtAl:2022:LREC3}, a collection of news articles with associated images.}, sort=n24news]{n24news}{N24News}{N24News}

\newabbreviation[category=nolong, description={The TREC dataset \citep{hovy-etal-2001-toward,li-roth-2002-learning}, designed for research in text retrieval and information extraction, includes a wide range of question types.}, sort=trec]{trec}{TREC}{TREC}

\newabbreviation[category=nolong, description={The Cora dataset \citep{cora}, a collection of scientific publications categorized into different classes, used for document classification and citation prediction.}, sort=cora]{cora}{Cora}{Cora}

\newabbreviation[category=nolong, description={The SVHN (Street View House Numbers) dataset \citep{netzer2011reading}, a real-world image dataset for developing machine learning and object recognition algorithms.}, sort=svhn]{svhn}{SVHN}{SVHN}

\newabbreviation[category=withdesc, description={The RoBERTa model \citep{roberta} with a base configuration, an optimized version of BERT that improves language understanding by carefully tuning hyperparameters and training with more data. Available pretrained on Hugging Face.}, sort=robertab]{robertab}{RoBERTa}{\texttt{roberta-base}}


\newglossaryentry{correspondence-parallel}{
  type=concepts,
  name={Correspondence-Parallel},
  text={correspondence-parallel},
  plural={correspondence-parallel operators},
  description={Operators that transform representation spaces independently using their respective sides of the correspondence $\Gamma$. Each space is processed separately using its own transformation: $\Pi_\Gamma^{\mathcal{X}}$ for space $\mathcal{X}$ and $\Pi_\Gamma^{\mathcal{Y}}$ for space $\mathcal{Y}$. Outputs live in auxiliary semantic coordinates that factor out extrinsic parameterization variations. These operators maximize modularity: one model's transformation does not require access to the other model's parameters or decoder. The independence enables efficient computation and deployment flexibility. See \Cref{ch:methodology}, \Cref{sec:operator-parallel} for formal definition and geometric interpretation.}
}

\newglossaryentry{correspondence-coupled}{
  type=concepts,
  name={Correspondence-Coupled},
  text={correspondence-coupled},
  plural={correspondence-coupled operators},
  description={Operators that jointly use both sides of correspondence $\Gamma$ to construct direct transformations between spaces. Unlike correspondence-parallel operators, these transformations require access to both spaces simultaneously: $T_\Gamma: \mathcal{X} \to \mathcal{Y}$ maps from space $\mathcal{X}$ to space $\mathcal{Y}$ by leveraging information from both sides. Outputs live in the target model's native (extrinsic) coordinates, enabling immediate use with the target decoder without additional projection. These operators trade modularity for decoder compatibility, making them suitable when preserving the target's coordinate system is critical. See \Cref{ch:methodology}, \Cref{sec:operator-coupled} for formal definition and when to prefer coupled over parallel operators.}
}

\newglossaryentry{semantic-coordinate}{
  type=concepts,
  name={Semantic Coordinate},
  text={semantic coordinate},
  plural={semantic coordinates},
  description={Representations that factor out extrinsic parameterization variations to reveal intrinsic functional structure anchored to semantic content. Achieved through correspondence-based transformations that break the symmetry of arbitrary coordinate system choices. While raw model representations live in extrinsic coordinates determined by architecture, initialization, and optimization trajectory, semantic coordinates expose the underlying semantic relationships the models compute independent of these parameterization choices. For example, relative representations (\Cref{ch:relative-representations}) transform activations into semantic coordinates by measuring angular relationships to anchor points, making representations directly comparable across models with different architectures. Contrasts with \emph{extrinsic/ambient coordinates} of native model representations. See \Cref{ch:methodology}, \Cref{sec:operator-parallel} for the functional perspective on why semantic coordinates enable cross-model alignment.}
}

\newglossaryentry{intrinsic-factor}{
  type=concepts,
  name={Intrinsic Factor},
  text={intrinsic factor},
  plural={intrinsic factors},
  description={Determinants of \emph{what function is learned} by a neural network, independent of how that function is parameterized. Primarily comprises: (1) \textbf{Data} $\mathcal{D}$---the semantic relationships, concept organization, and statistical structure present in training samples; (2) \textbf{Task objective} $\mathcal{L}_{\mathrm{task}}$---what semantic structure must be extracted to succeed (e.g., discriminative objectives that force models to learn rich semantic geometry to separate classes). When task objectives demand extraction of semantic structure from data, different parameterizations (even different architectures) tend to converge toward functionally similar solutions that capture this intrinsic structure, though expressed in incompatible coordinate systems. This convergence explains why correspondence-based alignment works: models trained on similar data and tasks learn similar functional relationships. See \Cref{ch:methodology}, \Cref{sec:neural-representations} for empirical evidence.}
}

\newglossaryentry{extrinsic-factor}{
  type=concepts,
  name={Extrinsic Factor},
  text={extrinsic factor},
  plural={extrinsic factors},
  description={Determinants of \emph{how a function is parameterized} by a neural network, affecting the coordinate system but not the underlying functional relationships. Comprises: (1) \textbf{Architectural choice}---CNNs vs.\ Transformers vs.\ ResNets, representing different parameterizations of function space with different inductive biases; (2) \textbf{Architectural details}---network depth, width, activation functions, normalization layers, structural choices affecting how functions are represented; (3) \textbf{Optimization dynamics}---initialization seed, learning rate, batch size, optimizer choice, determining which point in parameter space represents the learned function. Universal approximation theorems establish that different architectures can represent similar functions; when task objectives force extraction of semantic structure, different parameterizations converge to functionally similar solutions in incompatible coordinate systems. Correspondence breaks this extrinsic symmetry, enabling transformation between parameterizations. See \Cref{ch:methodology}, \Cref{sec:neural-representations} for the role of extrinsic factors in the functional perspective.}
}

\newglossaryentry{correspondence-concept}{
  type=concepts,
  name={Correspondence},
  text={correspondence},
  plural={correspondences},
  description={Semantic relationships between observation spaces that break the symmetry of arbitrary parameterization choices. Formally, a correspondence $\Gamma$ establishes semantic connections between samples, features, or distributional properties across domains (e.g., shared anchor points in \Cref{ch:relative-representations}, paired activations in \Cref{ch:semantic_alignment}, spectral relationships in \Cref{ch:lfm}). Correspondence serves as the fundamental primitive for representation alignment: it anchors parameterization-dependent coordinates to shared semantic content, revealing the intrinsic functional geometry (semantic relationships the models compute) while factoring out extrinsic parameterization (how those computations are represented). This enables transformation between models with different architectures, training procedures, or initialization seeds. The framework distinguishes two operator families based on how correspondence is used: correspondence-parallel operators (transform spaces independently) and correspondence-coupled operators (use both sides together). See \Cref{ch:methodology}, \Cref{sec:correspondence} for the central role of correspondence in the functional perspective.}
}

\newabbreviation{ao}{AO}{Anchor Optimization}

\newabbreviation[category=withoutdesc, sort=l1]{l1}{\ensuremath{L_1}}{Manhattan distance}

\newabbreviation[category=withoutdesc, sort=linf]{linf}{\ensuremath{L_\infty}}{Chebyshev distance}

\newabbreviation[category=withoutdesc, sort=gcn]{gcn}{GCN}{Graph Convolutional Network}

\newabbreviation[category=withoutdesc, sort=qkv]{qkv}{QKV}{Query-Key-Value}

\newglossaryentry{jaccard-similarity}{
  type=concepts,
  name={Jaccard Similarity},
  text={Jaccard similarity},
  description={A set-based similarity metric measuring the overlap between retrieved nearest-neighbor sets. Computed as the size of the intersection divided by the size of the union of two sets: $J(\mathcal{S}_1,\mathcal{S}_2) = \lvert\mathcal{S}_1 \cap \mathcal{S}_2\rvert / \lvert\mathcal{S}_1 \cup \mathcal{S}_2\rvert$. In retrieval tasks, quantifies how well the retrieved neighbors match the ground truth neighbors. Values range from 0 (no overlap) to 1 (perfect match). Higher values indicate better retrieval quality.}
}

\newglossaryentry{mrr}{
  type=concepts,
  name={Mean Reciprocal Rank},
  text={mean reciprocal rank},
  description={A ranking metric that quantifies the quality of retrieval by averaging the reciprocal rank of the first correct retrieval across queries. Computed as $\operatorname{MRR}(\mX,\mY) = \frac{1}{n}\sum_{i=1}^{n} \frac{1}{\operatorname{rank}(\vx_i,\mY)}$, where the rows $\vx_i$ of $\mX$ and $\vy_i$ of $\mY$ are $n$ paired representations and $\operatorname{rank}(\vx_i,\mY)$ is the position of the true match $\vy_i$ among the rows of $\mY$ ranked by similarity to $\vx_i$. Values range from 0 to 1, with higher values indicating that correct results appear earlier in rankings. Emphasizes the importance of top-ranked results.}
}

\newglossaryentry{cosine-similarity}{
  type=concepts,
  name={Cosine Similarity},
  text={cosine similarity},
  description={A metric measuring the angular alignment between vectors, computed as the dot product of normalized vectors: $\cos(\vx, \vy) = \frac{\vx^\top \vy}{\lVert \vx \rVert \lVert \vy \rVert}$. In representation alignment, quantifies how well transformed representations preserve directional relationships. Values range from -1 (opposite directions) to 1 (same direction), with 0 indicating orthogonality. Widely used in neural network similarity analysis as it is invariant to vector magnitude, focusing purely on orientation.}
}


==> glossaries/symbols.tex <==
\glsxtrnewsymbol[sort=Gamma, seealso={correspondence-concept}, description={Correspondence between observation spaces. In general $\Gamma \subseteq \mathcal{P}(\mathcal{O}_{\mathcal{X}}) \times \mathcal{P}(\mathcal{O}_{\mathcal{Y}})$ relates sets of observations; element-wise, $\Gamma \subseteq \mathcal{O}_{\mathcal{X}} \times \mathcal{O}_{\mathcal{Y}}$ pairs observations. $\Gamma_{\mathcal{X}}$, $\Gamma_{\mathcal{Y}}$ are its sides; a superscript or prime distinguishes several correspondences ($\Gamma^{\mathrm{seed}}$, $\Gamma^{\mathrm{boot}}$ in \cref{ch:bootstrapping}; $\Gamma'$); $\Gamma_\sharp$ is the correspondence lifted to functions by push-forward (\cref{ch:lfm}).}]{Corr}{\ensuremath{\Gamma}}

\glsxtrnewsymbol[sort=Pi, seealso={correspondence-parallel}, description={Correspondence-parallel operator family. Applied to a representation: $\Pi_\Gamma^{\mathcal{X}}(\bm{x})$.}]{OperatorParallel}{\ensuremath{\Pi}}

\glsxtrnewsymbol[sort=Tau, seealso={correspondence-coupled}, description={Correspondence-coupled operator family, $T_\Gamma: \mathcal{X} \to \mathcal{Y}$.}]{OperatorCoupled}{\ensuremath{T}}

\glsxtrnewsymbol[sort=Sigma, description={Correspondence-coupled same-space operator: the coupled operator when source and target space coincide, $\Sigma_\Gamma: \mathcal{X} \to \mathcal{X}$.}]{OperatorSameSpace}{\ensuremath{\Sigma}}

\glsxtrnewsymbol[sort=O, description={Observation space, the inputs of a model (images, texts, states, prompts). $\mathcal{O}_{\mathcal{X}}$ is the domain of the source model.}]{Obs}{\ensuremath{\mathcal{O}}}

\glsxtrnewsymbol[sort=o, description={An observation, $o \in \mathcal{O}$.}]{obs}{\ensuremath{o}}

\glsxtrnewsymbol[sort=D, description={Dataset, a finite set of observations, $\mathcal{D} \subset \mathcal{O}$.}]{Data}{\ensuremath{\mathcal{D}}}

\glsxtrnewsymbol[sort=X, description={Representation spaces: source, target and a third space.}]{Space}{\ensuremath{\mathcal{X}, \mathcal{Y}, \mathcal{Z}}}

\glsxtrnewsymbol[sort=x, description={A representation, $\bm{x} = E_{\mathcal{X}}(o) \in \mathcal{X}$; $\bm{y} = E_{\mathcal{Y}}(o') \in \mathcal{Y}$ on the target side.}]{RepVec}{\ensuremath{\bm{x}}}

\glsxtrnewsymbol[sort=X matrix, description={Representations stacked row-wise, $\bm{X} \in \mathbb{R}^{n \times d_{\mathcal{X}}}$ for $n$ samples; $\bm{Y}$ on the target side.}]{RepMat}{\ensuremath{\bm{X}}}

\glsxtrnewsymbol[sort=d, description={Dimension of $\mathcal{X}$; plain $d$ when only one space is involved.}]{DimLatent}{\ensuremath{d_{\mathcal{X}}}}

\glsxtrnewsymbol[sort=E, seealso={encoder}, description={Encoder, $E_{\mathcal{X}}: \mathcal{O} \to \mathcal{X}$.}]{Enc}{\ensuremath{E_{\mathcal{X}}}}

\glsxtrnewsymbol[sort=D decoder, seealso={decoder}, description={Decoder or task head of the model with representation space $\mathcal{X}$.}]{Dec}{\ensuremath{D_{\mathcal{X}}}}

\glsxtrnewsymbol[sort=F, description={Whole model with parameters $\theta$, $F_\theta = D \circ E$.}]{Model}{\ensuremath{F_\theta}}

\glsxtrnewsymbol[sort=A, description={Anchor set, a subset of observations; $\mathcal{A}_{\mathcal{X}}$ on one side.}]{Anchors}{\ensuremath{\mathcal{A}}}

\glsxtrnewsymbol[sort=a, description={Embedding of one anchor observation $a_j \in \mathcal{A}$, $\bm{a}_j = E_{\mathcal{X}}(a_j)$; $a'_j$ is its target-side counterpart, with embedding $\bm{a}'_j = E_{\mathcal{Y}}(a'_j)$.}]{AnchorEmb}{\ensuremath{\bm{a}_j}}

\glsxtrnewsymbol[sort=A matrix, description={Anchor embeddings stacked row-wise, $\bm{A}_{\mathcal{X}} \in \mathbb{R}^{K \times d_{\mathcal{X}}}$.}]{AnchorMat}{\ensuremath{\bm{A}_{\mathcal{X}}}}

\glsxtrnewsymbol[sort=K, description={Number of anchors, $K = \lvert\mathcal{A}\rvert$.}]{NumAnchors}{\ensuremath{K}}

\glsxtrnewsymbol[sort=sim, description={Similarity between representations; $\cos$ when it is the cosine similarity; a family $\operatorname{sim}_1,\dots,\operatorname{sim}_m$ when several are combined.}]{Sim}{\ensuremath{\operatorname{sim}}}

\glsxtrnewsymbol[sort=rel, description={Relative projection, $\operatorname{rel}(\bm{x}) = [\operatorname{sim}(\bm{x},\bm{a}_1),\dots,\operatorname{sim}(\bm{x},\bm{a}_K)] \in \mathbb{R}^K$; $\operatorname{rel}_{\mathcal{A}_{\mathcal{X}}}$ when the anchor set matters, $\operatorname{rel}_{\operatorname{sim}_i}$ under a specific similarity. $\bm{r} = \operatorname{rel}(\bm{x})$ is the relative representation; $\bm{X}_{\mathrm{rel}} = \bm{X}\bm{A}_{\mathcal{X}}^\top \in \mathbb{R}^{n \times K}$ stacks them.}]{RelProj}{\ensuremath{\operatorname{rel}}}

\glsxtrnewsymbol[sort=T linear, description={General linear map, orthogonal map, permutation or coupling matrix, and bias.}]{LinMap}{\ensuremath{\bm{T}, \bm{R}, \bm{P}, \bm{b}}}

\glsxtrnewsymbol[sort=tau, description={A transformation $\tau \in \mathcal{T}$ from a class $\mathcal{T}$.}]{TransfClass}{\ensuremath{\tau \in \mathcal{T}}}

\glsxtrnewsymbol[sort=n, description={Number of samples.}]{NumSamples}{\ensuremath{n}}

\glsxtrnewsymbol[sort=L loss, description={Loss; $\mathcal{L}_{\mathrm{task}}$ is the task objective.}]{Loss}{\ensuremath{\mathcal{L}}}

\glsxtrnewsymbol[sort=R regularizer, description={Regularizer.}]{Reg}{\ensuremath{\mathcal{R}}}

\glsxtrnewsymbol[sort=M manifold, description={Manifold; in \cref{ch:lfm}, $\mathcal{M} \subset \mathcal{X}$ and $\mathcal{N} \subset \mathcal{Y}$.}]{Manifold}{\ensuremath{\mathcal{M}}}

\glsxtrnewsymbol[sort=f layer, description={Layer $f_\ell$ of a network with $L$ layers; $\ell$ is the layer index.}]{Layer}{\ensuremath{f_\ell, \ell, L}}

